Holistic Guidance for Occluded Person Re-Identification

In real-world video surveillance applications, person re-identification (ReID) suffers from the effects of occlusions and detection errors. Despite recent advances, occlusions continue to corrupt the features extracted by state-of-art CNN backbones, and thereby deteriorate the accuracy of ReID systems. To address this issue, methods in the literature use an additional costly process such as pose estimation, where pose maps provide supervision to exclude occluded regions. In contrast, we introduce a novel Holistic Guidance (HG) method that relies only on person identity labels, and on the distribution of pairwise matching distances of datasets to alleviate the problem of occlusion, without requiring additional supervision. Hence, our proposed student-teacher framework is trained to address the occlusion problem by matching the distributions of between- and within-class distances (DCDs) of occluded samples with that of holistic (non-occluded) samples, thereby using the latter as a soft labeled reference to learn well separated DCDs. This approach is supported by our empirical study where the distribution of between- and within-class distances between images have more overlap in occluded than holistic datasets. In particular, features extracted from both datasets are jointly learned using the student model to produce an attention map that allows separating visible regions from occluded ones. In addition to this, a joint generative-discriminative backbone is trained with a denoising autoencoder, allowing the system to self-recover from occlusions. Extensive experiments on several challenging public datasets indicate that the proposed approach can outperform state-of-the-art methods on both occluded and holistic datasets

==> latex/duplicates.tex <==
{gao2020pose, occ_pose_match}  --> gao2020pose

{partial1, occ_deeprecons}  --> partial1

{occ_foreground, partial2}  --> partial2


{hacnn, li2018harmonious}  --> li2018harmonious


{lomo, liao2015person} -- > liao2015person

{dukeDUPLICATED, duke2, duke}  --> dukeDUPLICATED


{song2018mask, maskguided}  --> song2018mask

{bilinear, suh2018part, part_alighned}  --> suh2018part



{sun2018beyond, partbased, part_pooling, sun2018beyondDUPLICATED}  --> sun2018beyond


{higherorder, occ_highorder, horeid}  --> higherorder


{zhao2017deeply, deeppartaligned, partaligned, person_iccv}   --> zhao2017deeply


{zheng2015scalable, market}  -> zheng2015scalable

{teacherstudent, occ_stuteac}  --> teacherstudent
